Benchmarking Middle-Trained Language Models for Neural Search

Middle training methods aim to bridge the gap between the Masked Language Model (MLM) pre-training and the final finetuning for retrieval. Recent models such as CoCondenser, RetroMAE, and LexMAE argue that the MLM task is not sufficient enough to pre-train a transformer network for retrieval and hence propose various tasks to do so. Intrigued by those novel methods, we noticed that all these models used different finetuning protocols, making it hard to assess the benefits of middle training. We propose in this paper a benchmark of CoCondenser, RetroMAE, and LexMAE, under the same finetuning conditions. We compare both dense and sparse approaches under various finetuning protocols and middle training on different collections (MS MARCO, Wikipedia or Tripclick). We use additional middle training baselines, such as a standard MLM finetuning on the retrieval collection, optionally augmented by a CLS predicting the passage term frequency. For the sparse approach, our study reveals that there is almost no statistical difference between those methods: the more effective the finetuning procedure is, the less difference there is between those models. For the dense approach, RetroMAE using MS MARCO as middle-training collection shows excellent results in almost all the settings. Finally, we show that middle training on the retrieval collection, thus adapting the language model to it, is a critical factor. Overall, a better experimental setup should be adopted to evaluate middle training methods. Code available at https://github.com/naver/splade/tree/benchmarch-SIGIR23

==> tables/models.tex <==
% To change the table size, act on the resizebox argument `0.8`.
\begin{table}[ht]
\centering
\caption{Models used and their characteristics (REMOVE IT?)}
\resizebox{0.5\textwidth}{!}{

\begin{tabular}{c|c|c|c}
\toprule
\textbf{Model} & \textbf{initial LM} &\textbf{training data} & \textbf{dense/sparse} \\
\midrule
distilbert & BERT &Wikibook  & N/A \\
BERT  & N/A &Wikibook  &  N/A \\
BERT MS & BERT &MSMARCO  & N/A \\
BERT MS CLS & BERT&  MSMARCO    & dense\\
coCondenser-ms & BERT&  MSMARCO    & dense\\
RetroMAE & BERT&  Wikibook  &   dense\\
LexMAE & BERT&  MSMARCO  &   sparse\\
\bottomrule
\end{tabular}
}
\label{tab:models}
\end{table}


==> tables/queriessparse.tex <==
    % To change the table size, act on the resizebox argument `0.8`.
\begin{table*}[ht]
\centering
\caption{ 100K queries (sparse distil)
Overall effectiveness of the models.
The best results are highlighted in boldface.
Superscripts denote significant differences in paired Student's t-test with $p \le 0.0035$.
}
\resizebox{0.8\textwidth}{!}{
\begin{tabular}{c|c|c|c|c|c|c|c}
\toprule
\textbf{\#}
& \textbf{Model}
& \textbf{MRR@10}
& \textbf{NDCG@10}
& \textbf{TR19MRR@10}
& \textbf{TR19NDCG@10}
& \textbf{TR20MRR@10}
& \textbf{TR20NDCG@10} \\
\midrule
a &
distilbert &
37.6\hphantom{$^{bcdef}$} &
72.2\hphantom{$^{bcdef}$} &
67.3\hphantom{$^{bcdef}$} \\
b &
bertms &
38.4$^{a}$\hphantom{$^{cdef}$} &
72.6\hphantom{$^{acdef}$} &
70.3\hphantom{$^{acdef}$} \\
c &
bertmscls &
38.7$^{a}$\hphantom{$^{bdef}$} &
72.5\hphantom{$^{abdef}$} &
\textbf{72.0}$^{a}$\hphantom{$^{bdef}$} \\
d &
cocondenser &
38.9$^{ae}$\hphantom{$^{bcf}$} &
\textbf{72.9}\hphantom{$^{abcef}$} &
71.1$^{a}$\hphantom{$^{bcef}$} \\
e &
RetroMAE &
38.2\hphantom{$^{abcdf}$} &
72.7\hphantom{$^{abcdf}$} &
69.7\hphantom{$^{abcdf}$} \\
f &
LexMAE &
\textbf{39.3}$^{abe}$\hphantom{$^{cd}$} &
72.8\hphantom{$^{abcde}$} &
70.3\hphantom{$^{abcde}$} \\
\bottomrule
\end{tabular}
}
\label{tab:results}
\end{table*}


==> tables/sparse_distil_1neg.tex <==
% To change the table size, act on the resizebox argument `0.8`.
\begin{table*}[ht]
\centering
\caption{ 
Evaluation for the dense, distillation, 1 negative settings
%Overall effectiveness of the models.
%The best results are highlighted in boldface.
%Superscripts denote significant differences in paired Student's t-test with $p \le 0.0033$.
}

\resizebox{0.8\textwidth}{!}{
\begin{tabular}{c|c|c|c|c|c|c|c}
\toprule
\textbf{\#}
& \textbf{Model}
& \textbf{MRR@10}
& \textbf{NDCG@10}
& \textbf{MRR@10}
& \textbf{NDCG@10}
& \textbf{MRR@10}
& \textbf{NDCG@10} \\
\midrule
a &
distilbert &
37.7\hphantom{$^{bcdef}$} &
%44.1\hphantom{$^{bcdef}$} &
%97.3\hphantom{$^{bcdef}$} &
\textbf{73.8}\hphantom{$^{bcdef}$} &
%94.1\hphantom{$^{bcdef}$} &
69.8\hphantom{$^{bcdef}$} \\
b &
bert &
37.8\hphantom{$^{acdef}$} &
%44.3\hphantom{$^{acdef}$} &
%96.9\hphantom{$^{acdef}$} &
72.9\hphantom{$^{acdef}$} &
%92.3\hphantom{$^{acdef}$} &
69.1\hphantom{$^{acdef}$} \\
c &
betmscls &
38.4\hphantom{$^{abdef}$} &
%45.0$^{ab}$\hphantom{$^{def}$} &
%\textbf{98.4}\hphantom{$^{abdef}$} &
71.7\hphantom{$^{abdef}$} &
%93.1\hphantom{$^{abdef}$} &
70.7\hphantom{$^{abdef}$} \\
d &
cocondenser &
\textbf{38.6}$^{ab}$\hphantom{$^{cef}$} &
%\textbf{45.2}$^{ab}$\hphantom{$^{cef}$} &
%96.9\hphantom{$^{abcef}$} &
73.6\hphantom{$^{abcef}$} &
%\textbf{95.4}\hphantom{$^{abcef}$} &
71.8\hphantom{$^{abcef}$} \\
e &
retroMAE &
38.1\hphantom{$^{abcdf}$} &
%44.6\hphantom{$^{abcdf}$} &
%97.3\hphantom{$^{abcdf}$} &
73.1\hphantom{$^{abcdf}$} &
%94.5\hphantom{$^{abcdf}$} &
70.1\hphantom{$^{abcdf}$} \\
f &
lexmae &
38.4\hphantom{$^{abcde}$} &
%45.0$^{a}$\hphantom{$^{bcde}$} &
%96.9\hphantom{$^{abcde}$} &
73.8\hphantom{$^{abcde}$} &
%94.1\hphantom{$^{abcde}$} &
\textbf{72.0}\hphantom{$^{abcde}$} \\
\bottomrule
\end{tabular}
}
\label{tab:results}
\end{table*}


==> tables/sparse_distil_32neg.tex <==
% To change the table size, act on the resizebox argument `0.8`.
\begin{table*}[ht]
\centering
\caption{
SPARSE DISTL 32 NEG
}
\resizebox{0.8\textwidth}{!}{
\begin{tabular}{c|c|c|c|c|c|c|c}
\toprule
\textbf{\#}
& \textbf{Model}
& \textbf{MRR@10}
& \textbf{NDCG@10}
& \textbf{MRR@10}
& \textbf{NDCG@10}
& \textbf{MRR@10}
& \textbf{NDCG@10} \\
\midrule
a &
distilbert &
39.1\hphantom{$^{bcdefg}$} &
45.4\hphantom{$^{bcdefg}$} &
95.7\hphantom{$^{bcdefg}$} &
73.0\hphantom{$^{bcdefg}$} &
\textbf{95.4}\hphantom{$^{bcdefg}$} &
72.0\hphantom{$^{bcdefg}$} \\
b &
BERT &
39.1\hphantom{$^{acdefg}$} &
45.5\hphantom{$^{acdefg}$} &
96.1\hphantom{$^{acdefg}$} &
\textbf{73.6}\hphantom{$^{acdefg}$} &
94.5\hphantom{$^{acdefg}$} &
71.3\hphantom{$^{acdefg}$} \\
c &
BERT-MS &
39.4\hphantom{$^{abdefg}$} &
45.9\hphantom{$^{abdefg}$} &
\textbf{97.3}\hphantom{$^{abdefg}$} &
71.2\hphantom{$^{abdefg}$} &
94.4\hphantom{$^{abdefg}$} &
\textbf{72.4}\hphantom{$^{abdefg}$} \\
d &
BERT-MS-CLS &
39.7\hphantom{$^{abcefg}$} &
46.2$^{ab}$\hphantom{$^{cefg}$} &
95.0\hphantom{$^{abcefg}$} &
71.9\hphantom{$^{abcefg}$} &
95.0\hphantom{$^{abcefg}$} &
72.4\hphantom{$^{abcefg}$} \\
e &
cocondenser &
39.6\hphantom{$^{abcdfg}$} &
46.1$^{ab}$\hphantom{$^{cdfg}$} &
97.3\hphantom{$^{abcdfg}$} &
72.4\hphantom{$^{abcdfg}$} &
95.0\hphantom{$^{abcdfg}$} &
71.7\hphantom{$^{abcdfg}$} \\
f &
retroMAE &
39.3\hphantom{$^{abcdeg}$} &
45.8\hphantom{$^{abcdeg}$} &
97.3\hphantom{$^{abcdeg}$} &
71.9\hphantom{$^{abcdeg}$} &
94.6\hphantom{$^{abcdeg}$} &
70.9\hphantom{$^{abcdeg}$} \\
g &
LexMAE &
\textbf{39.8}$^{ab}$\hphantom{$^{cdef}$} &
\textbf{46.3}$^{ab}$\hphantom{$^{cdef}$} &
94.4\hphantom{$^{abcdef}$} &
72.2\hphantom{$^{abcdef}$} &
95.3\hphantom{$^{abcdef}$} &
72.1\hphantom{$^{abcdef}$} \\
\bottomrule
\end{tabular}
}
\label{tab:results}
\end{table*}
%distilbert 0.456898
%bert 0.456777
%lexmae 0.45561
%retromae ms  0.405828  ??
%coco 0.464452
%bert ms 0.458855
%retro 0.458875
%bert ms cls running
